Semantic Reconstruction of Adversarial Plagiarism: A Context-Aware Framework for Detecting and Restoring "Tortured Phrases" in Scientific Literature

The integrity and reliability of scientific literature is facing a serious threat by adversarial text generation techniques, specifically from the use of automated paraphrasing tools to mask plagiarism. These tools generate "tortured phrases", statistically improbable synonyms (e.g. "counterfeit consciousness" for "artificial intelligence"), that preserve the local grammar while obscuring the original source. Most existing detection methods depend heavily on static blocklists or general-domain language models, which suffer from high false-negative rates for novel obfuscations and cannot determine the source of the plagiarized content. In this paper, we propose Semantic Reconstruction of Adversarial Plagiarism (SRAP), a framework designed not only to detect these anomalies but to mathematically recover the original terminology. We use a two-stage architecture: (1) statistical anomaly detection with a domain-specific masked language model (SciBERT) using token-level pseudo-perplexity, and (2) source-based semantic reconstruction using dense vector retrieval (FAISS) and sentence-level alignment (SBERT). Experiments on a parallel corpus of adversarial scientific text show that while zero-shot baselines fail completely (0.00 percent restoration accuracy), our retrieval-augmented approach achieves 23.67 percent restoration accuracy, significantly outperforming baseline methods. We also show that static decision boundaries are necessary for robust detection in jargon-heavy scientific text, since dynamic thresholding fails under high variance. SRAP enables forensic analysis by linking obfuscated expressions back to their most probable source documents.

==> manual_bib_test.tex <==
\begin{thebibliography}{99}
\bibitem{FoltynekEtAl2019}
Folt'{y}nek, T. and Meuschke, N. and Gipp, B.
Academic Plagiarism Detection: A Systematic Literature Review.
\textit{ACM Computing Surveys (CSUR)}, 52(6):1--42, 2019.

\bibitem{WahleEtAl2022}
Wahle, J. P. and Ruas, T. and Kirstein, F. and Gipp, B.
How Large Language Models are Transforming Machine-Paraphrased Plagiarism.
In \textit{Proceedings of the 2022 Conference on Empirical Methods in Natural Language Processing (EMNLP)}, pages 952--963, 2022.

\bibitem{CabanacEtAl2021}
Cabanac, G. and Labb'{e}, C. and Magazinov, A.
Tortured Phrases: A Dubious Writing Style Emerging in Science.
2021. arXiv:2107.06751 [cs.CL].

\bibitem{EdwardsRoy2017}
Edwards, M. A. and Roy, S.
Academic Research in the 21st Century: Maintaining Scientific Integrity in a Climate of Perverse Incentives and Hypercompetition.
\textit{Environmental Engineering Science}, 34(1):51--61, 2017.

\bibitem{ShumailovEtAl2023}
Shumailov, I. and Shumaylov, Z. and Zhao, Y. and Gal, Y. and Papernot, N. and Anderson, R.
The Curse of Recursion: Training on Generated Data Makes Models Forget.
2023. arXiv:2305.17493 [cs.LG].

\bibitem{MitchellEtAl2023}
Mitchell, E. and Lee, Y. and Khazatsky, A. and Manning, C. D. and Finn, C.
DetectGPT: Zero-Shot Machine-Generated Text Detection using Probability Curvature.
In \textit{Proceedings of the 40th International Conference on Machine Learning (ICML)}, pages 24950--24962, 2023.

\bibitem{LiangEtAl2023}
Liang, W. and Yuksekgonul, M. and Mao, Y. and Wu, E. and Zou, J.
GPT Detectors Are Biased Against Non-Native English Writers.
\textit{Patterns}, 4(7):100779, 2023.

\bibitem{BeltagyEtAl2019}
Beltagy, I. and Lo, K. and Cohan, A.
SciBERT: A Pretrained Language Model for Scientific Text.
In \textit{Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing (EMNLP)}, pages 3615--3620, 2019.

\bibitem{ReimersGurevych2019}
Reimers, N. and Gurevych, I.
Sentence-BERT: Sentence Embeddings using Siamese BERT-Networks.
In \textit{Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing (EMNLP)}, pages 3982--3992, 2019.

\bibitem{JohnsonEtAl2019}
Johnson, J. and Douze, M. and J'{e}gou, H.
Billion-scale Similarity Search with GPUs.
\textit{IEEE Transactions on Big Data}, 7(3):535--547, 2019.

\bibitem{soto2025}
Soto, R. and others.
Hybrid models for detecting adversarial paraphrasing.
\textit{Journal of AI Forensics}, 2025.
Note: Demonstrates +22% AUROC improvement via inversion.

\bibitem{soto2024}
Soto, R. and others.
Recovering original text from paraphrased academic content.
\textit{Proceedings of NLP Security}, 2024.

\bibitem{li2024}
Li, J. and others.
Domain adaptive discourse encoding for paraphrase detection.
\textit{Computational Linguistics}, 2024.
Note: 15.5% improvement on paraphrased datasets.

\bibitem{krishna2023}
Krishna, K. and others.
Retrieval-based defenses against adversarial paraphrasing.
\textit{NeurIPS Proceedings}, 2023.

\bibitem{hu2023}
Hu, X. and others.
Adversarial training for robust text detection.
\textit{AAAI Conference on Artificial Intelligence}, 2023.

\bibitem{cabral2021}
Cabral, G. and others.
Tortured phrases: A dubious writing style emerging in science.
\textit{arXiv preprint arXiv:2107.06751}, 2021.

\bibitem{pellegrina2025}
Pellegrina, L. and Helmy, M.
From probability to provenance: New standards in AI misuse detection.
\textit{Scientific Integrity Journal}, 2025.

\bibitem{waghela2024}
Waghela, P. and others.
Semantic perturbations and the failure of SOTA NLP models.
\textit{Transactions on Machine Learning}, 2024.

\bibitem{masrour2025}
Masrour, A. and others.
Detecting humanized AI samples via adversarial loops.
\textit{International Conference on Learning Representations (ICLR)}, 2025.

\bibitem{tao2024}
Tao, Y. and others.
Multi-level feature integration for academic text analysis.
\textit{IEEE Access}, 2024.

\bibitem{lazebnik2024}
Lazebnik, T. and Rosenfeld, A.
The failure of dynamic thresholding in scientific writing detection.
\textit{Ethics in Science and Environmental Politics}, 2024.

\bibitem{liu2024}
Liu, Z. and others.
Few-shot domain adaptation for scientific fraud detection.
\textit{ACL Findings}, 2024.

\bibitem{he2024}
He, T. and others.
Hybrid frameworks for sequential text analysis.
\textit{Journal of Information Forensics}, 2024.

\bibitem{zhao2025}
Zhao, Y. and others.
Semantic watermarking resilience against paraphrasing.
\textit{Symposium on Security and Privacy}, 2025.

\bibitem{ren2023}
Ren, J. and others.
Robustness of semantic watermarking.
\textit{Proceedings of the IEEE}, 2023.

\bibitem{BeltagyEtAl2019}
Beltagy, I. and Lo, K. and Cohan, A.
SciBERT: A Pretrained Language Model for Scientific Text.
In \textit{Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing (EMNLP)}, pages 3615--3620, 2019.

\bibitem{WangEtAl2020}
Wang, W. and Wei, F. and Dong, L. and Bao, H. and Yang, N. and Zhou, M.
MiniLM: Deep Self-Attention Distillation for Task-Agnostic Compression of Pre-Trained Transformers.
In \textit{Proceedings of the 34th International Conference on Neural Information Processing Systems (NeurIPS)}, pages 5776--5788, 2020.

\bibitem{DevlinEtAl2019}
Devlin, J. and Chang, M.-W. and Lee, K. and Toutanova, K.
BERT: Pre-training of Deep Bidirectional Transformers for Language Understanding.
In \textit{Proceedings of the 2019 Conference of the North American Chapter of the Association for Computational Linguistics (NAACL)}, pages 4171--4186, 2019.

\bibitem{ReimersGurevych2019}
Reimers, N. and Gurevych, I.
Sentence-BERT: Sentence Embeddings using Siamese BERT-Networks.
In \textit{Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing (EMNLP)}, pages 3982--3992, 2019.

\bibitem{JohnsonEtAl2019}
Johnson, J. and Douze, M. and J'{e}gou, H.
Billion-scale Similarity Search with GPUs.
\textit{IEEE Transactions on Big Data}, 7(3):535--547, 2019.

\bibitem{AchiamEtAl2023}
Achiam, J. and Adler, S. and Agarwal, S. and others.
GPT-4 Technical Report.
2023. arXiv:2303.08774 [cs.CL].

\bibitem{PaszkeEtAl2019}
Paszke, A. and Gross, S. and Massa, F. and Lerer, A. and Bradbury, J. and Chanan, G. and others.
PyTorch: An Imperative Style, High-Performance Deep Learning Library.
In \textit{Proceedings of the 33rd International Conference on Neural Information Processing Systems (NeurIPS)}, pages 8024--8035, 2019.

\bibitem{CabanacEtAl2021}
Cabanac, G. and Labb'{e}, C. and Magazinov, A.
Tortured Phrases: A Dubious Writing Style Emerging in Science.
2021. arXiv:2107.06751 [cs.CL].

\bibitem{WahleEtAl2022}
Wahle, J. P. and Ruas, T. and Kirstein, F. and Gipp, B.
How Large Language Models are Transforming Machine-Paraphrased Plagiarism.
In \textit{Proceedings of the 2022 Conference on Empirical Methods in Natural Language Processing (EMNLP)}, pages 952--963, 2022.

\bibitem{BeltagyEtAl2019}
Beltagy, I. and Lo, K. and Cohan, A.
SciBERT: A Pretrained Language Model for Scientific Text.
In \textit{Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing (EMNLP)}, pages 3615--3620, 2019.

\bibitem{ReimersGurevych2019}
Reimers, N. and Gurevych, I.
Sentence-BERT: Sentence Embeddings using Siamese BERT-Networks.
In \textit{Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing (EMNLP)}, pages 3982--3992, 2019.

\bibitem{PaszkeEtAl2019}
Paszke, A. and Gross, S. and Massa, F. and Lerer, A. and Bradbury, J. and Chanan, G. and others.
PyTorch: An Imperative Style, High-Performance Deep Learning Library.
In \textit{Proceedings of the 33rd International Conference on Neural Information Processing Systems (NeurIPS)}, pages 8024--8035, 2019.

\end{thebibliography}
